Joint 3D Human Shape Recovery and Pose Estimation from a Single Image with Bilayer Graph

The ability to estimate the 3D human shape and pose from images can be useful in many contexts. Recent approaches have explored using graph convolutional networks and achieved promising results. The fact that the 3D shape is represented by a mesh, an undirected graph, makes graph convolutional networks a natural fit for this problem. However, graph convolutional networks have limited representation power. Information from nodes in the graph is passed to connected neighbors, and propagation of information requires successive graph convolutions. To overcome this limitation, we propose a dual-scale graph approach. We use a coarse graph, derived from a dense graph, to estimate the human's 3D pose, and the dense graph to estimate the 3D shape. Information in coarse graphs can be propagated over longer distances compared to dense graphs. In addition, information about pose can guide to recover local shape detail and vice versa. We recognize that the connection between coarse and dense is itself a graph, and introduce graph fusion blocks to exchange information between graphs with different scales. We train our model end-to-end and show that we can achieve state-of-the-art results for several evaluation datasets.

==> sections/discussion.tex <==
\section{Discussion and Future Work} %\Note{SC: do we need this?}
\label{sec:discussion}

Compared to other approaches our method relies on 2D joint information as input, to determine the local image regions which are encoded and concatenated to the joints in the joint branch. In the supplementary material to this paper we evaluate the performance when the 2D joint estimates are automatically detected, e.g. from~\cite{cao2018openpose}. 

Some poses, and partial occlusions remain challenging. Thus far we have focused on single images as our input.  We would like to extend our work to take both single and multi-view images as input to improve performance. Furthermore, 3D reconstruction of objects from images in general, not only humans, is an interesting research direction. 

%We have presented a method which can propagate global and local information for improved 3D shape and pose reconstruction. To some extent we overcome the limitation of GCNs discussed in~\cite{Ci_2019_ICCV, Zhao_2019_CVPR} by proposing two branches for graphs at different scales, which exchange information by graph fusion. Our emphasis is on connectivity learning, i.e., how information can be shared to efficiently propagate over the graphs. The methods proposed by~\cite{Ci_2019_ICCV, Zhao_2019_CVPR} place more emphasis on feature learning instead.

%Although we focused on single images as our input, some methods, .e.g,~\cite{pifuSHNMKL19}, can handle both. We would like to extend our work to take both single and multi-view images as input. 

%We have presented our work in the context of 3D human shape and pose, however the multi-scale concept is applicable to general 3D object reconstruction from images. Coarse-to-fine approaches are common in computer graphics, for example in progressive representations which add detail with each level. The iterative approaches described in~\cite{meshrcnn, Wang_2018_ECCV, Wen_2019_ICCV} already use a coarse to fine approach. A similar approach would be preferable in this context, where the coarse level captures global pose, and subsequent levels add more detail to the shape. To reduce the number of learnable parameters, an interesting direction would be to explore recurrent models. 

%To train the network we rely on several different loss formulations that are added together. It's important that the losses all are scaled appropriately to ensure stable training. Recent work~\cite{Sener_2018_NIPS} proposes to compute a gradient which results in a more optimal adjustment of parameters while considering multiple tasks. The different losses can be considered different tasks, and a similar approach can be applied. 

%Finally, Reconstruct more detail in the non-parametric meshes, e.g.,~\cite{pifuSHNMKL19}.



==> sections/experiments.tex <==


\textbf{XIN:}

\textbf{TODO list of Ablation study:}
\begin{enumerate}
\item  For efficiency of local feature:
    \begin{enumerate}
        \item concat local feature and global feature for GraphCMR
        \item one GFB to fuse local and global feature before GraphCRM
    \end{enumerate}    
\item For efficiency of GFB:
    \begin{enumerate}
        \item one GFB before joint branch and mesh branch
    \item one GFB after joint branch and mesh branch 
    \item share GFB for each layer         
    \item remove GFB 
    \item remove GFB and share weights with/without local feature
    \end{enumerate}
\item For the generality of dual-path: make joint-branch only performs as global message passing.(vs. on-local)
    \begin{enumerate}
        \item remove loss for joint-branch
        \item remove loss and the local feature input for joint-branch.
    \end{enumerate}
\end{enumerate}
\textbf{Analysis of the framework}
\begin{enumerate}
    \item Perspective from 3D reconstruction: 
    \begin{enumerate}
       \item 3D Mesh -- 3D joints -- 2D joints mapping(semantic alignment); \\
        Different from Mesh rcnn, Pixel2Mesh which projects 3D points to 2D pixel with known camera parameters for alignment.
        \item Adaptive adjacent matrix in GFB learns the mapping between 3D Mesh -- 2D joints 
        \item sharing weights between two branches: coarse transformation learnt from high-level graph can be consistent with the fine transformation learnt from low-level graph. \\
    Next step: can we learn coarse transformation and then apply it to low-level graph directly? \\
    Only sharing the weights(or we can say one branch with two forward and back-propagation), no fusion. 
        \end{enumerate}
    \item Perspective from dual-path GCN: 
    \begin{enumerate}
        \item Speedup the convergence;
        \item Verify whether dual-path can be useful in general:
            Remove the supervision(loss) from joint-branch.\\
            Remove the input/use the same global feature for joint branch without supervision. 
        \item Supervision for both branch 
    \end{enumerate}
\end{enumerate}


\section{Emperical Evaluations}
\label{sec:experiments}

We have evaluated our proposed method and present the results in this section. We will first briefly discuss the datasets we used, training procedure and implementation.

\subsection{Datasets}
The training data consists of several datasets, some of which provide a combination of 2D and 3D supervision, whereas others provide only 2D keypoint supervision. Next, we briefly describe each dataset.

\noindent \textbf{Human 3.6M} This indoor 3D dataset~\cite{h36m_pami, IonescuSminchisescu11} comprises eleven subjects performing 17 common scenarios, e.g. sitting down, talking on the phone. The training data contains ground truth 2D joints, 3D joints, and SMPL (pose and shape) parameters. The entire dataset contains 3.6M images. For training we only have access to subjects 1, 5, 6, 7, and 8 for a total 1.55M images. Subjects 9 and 11 are held out for evaluation (about 0.5M images). \\
\textbf{UP-3D} Unite the People 3D~\cite{Lassner:UP:2017} consists of images with annotations by humans doing sports and other miscellaneous activities. Besides ground truth 2d keypoints, SMPL fits have been performed on the 2D keypoints to produce ground truth SMPL parameters. About 7K images are used for training, and 639 held out for evaluation. \\
\textbf{LSP} Leeds Sports Pose~\cite{Johnson10} contains 2K images with 2D joint annotations of people playing sports. We use 1000 images for training, and 1000 for evaluation. \\
\textbf{COCO} Common Object in COntext~\cite{MSCOCO_ECCV_2014} also contains images of people annotated with 2D keypoints. About 28K images are used for training. We do not evaluate for this dataset. \\
\textbf{MPII} MPII Human Pose dataset contains images with annotated body joints of people performing 410 different activities~\cite{andriluka14cvpr}. We use about 15K training images from this dataset, and do not evaluate on this dataset.

The datasets have different 2D annotations. We have selected the 12 joint annotations which they all have in common. The joint GCN uses those twelve joints to define its graph structure.

%\textbf{We need to say that we have specific evaluation datasets for each of above?}. Discuss how the nr of joints per dataset differs, and we pick those which are the same among all. This is important for training the joint branch. Elaborate!!!

%\paragraph{Dataset Pre-processing} Anything?
%We train on the same datasets as Graph CMR. Describe the difference in Human 3.6M joints versus SMPL joints. Describe the transformation we apply to the ground truth data in order to make all data more consistent.
\begin{table*}[thb!]
\centering
\scriptsize
\begin{tabular}{l | c | c | c | c | c | c | c | c | c | c | c | c | c | c }
  \hline
   & \multicolumn{4}{|c|}{H36M P1} & \multicolumn{4}{|c|}{H36M P2} & \multicolumn{2}{|c|}{UP-3D} & \multicolumn{4}{|c}{LSP} \\
  \hline
     \multirow{2}{*}{Methods} & MPJPE & RE & MPJPE & RE & MPJPE & RE & MPJPE & RE & Sh. Err. & Sh. Err. & \multirow{2}{*}{FB Acc.} & \multirow{2}{*}{FB F1} & \multirow{2}{*}{Parts Acc.} & \multirow{2}{*}{Parts F1} \\
      & (np) & (np) & (p) & (p) & (np) & (np) & (p) & (p) & (np) & (p) & & & & \\
%  \hline
%    Methods & \multicolumn{7}{c}{} \\
  \hline
    HMR~\cite{hmrKanazawa17} & - & - & 88.0 & 58.1 & - & - & - & 56.8 & - & - & 91.67 & 0.87 & 87.12 & 0.60 \\  
    \hdashline
    G-CMR~\cite{kolotouros2019cmr} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3 & 71.9 & 50.1 & - & - & 91.46 & 0.87 & 88.69 & 0.66 \\
    \hdashline
    MFL~\cite{Kolotouros_2019_ICCV} & - & - & - & - & - & - & - & 41.1 & - & - & 91.83 & 0.87 & 89.41 & 0.68 \\
    \hdashline
    Ours & \textbf{62.4} & \textbf{37.7} & \textbf{65.9} & \textbf{41.2} & \textbf{59.7} & \textbf{36.6} & \textbf{64.1} & \textbf{40.4} & \textbf{66.3} & \textbf{66.4} & \textbf{93.09} & \textbf{0.89} & \textbf{90.90} & \textbf{0.74} \\
  \hline
%  \hline
%    \multicolumn{2}{l|}{HMR~\cite{hmrKanazawa17}} & - & - & - & - & - & 91.67 & 87.12 \\  
%    \multicolumn{2}{l|}{} & 88.0 & 58.1 & - & 56.8 & - & 0.87 & 0.60 \\
%    \hdashline
%    \multicolumn{2}{l|}{G-CMR~\cite{kolotouros2019cmr}} & 75.0 & 51.2 & 72.7 & 49.3 & - & 91.46 & 88.69 \\
%    \multicolumn{2}{l|}{} & 74.7 & 51.9 & 71.9 & 50.1 & - & 0.87 & 0.66 \\
%    \hdashline
%    \multicolumn{2}{l|}{G-CMR~\cite{kolotouros2019cmr}\(^\dagger\)} & 74.0 & 54.9 & 73.5 & 54.0 & 152.6 & 90.52 & 87.90 \\
%    \multicolumn{2}{l|}{} & 77.5 & 57.6 & 75.6 & 56.1 & 200.3 & 0.85 & 0.65 \\
%    \hdashline
%    \multicolumn{2}{l|}{MFL~\cite{Kolotouros_2019_ICCV}} & - & - & - & - & - & 91.83 & 89.41 \\
%    \multicolumn{2}{l|}{} & - & - & - & 41.1 & - & 0.87 & 0.68 \\
%    \hdashline
%    \multicolumn{2}{l|}{Ours} & \textbf{62.4} & \textbf{37.7} & \textbf{59.7} & \textbf{36.6} & \textbf{66.3} & \textbf{93.09} & \textbf{90.90} \\
%    \multicolumn{2}{l|}{} & 65.9 & 41.2 & 64.1 & 40.4 & 66.4 & \textbf{0.89} & \textbf{0.74} \\
%  \hline
\end{tabular}
\caption{Results for evaluation on Human 3.6M, LSP and Up-3D datasets. Error metrics MPJPE and RE are defined in~\cite{Zhou:2019:MMHM}. For evaluation datasets H36M P1, P2 and UP-3D the errors metrics are reported for non-parametric (np) and parametric SMPL meshes (p). For LSP evaluation we report accuracy and F1 score. Our proposed method outperforms the state of the art, including the iterative regression followed by optimization~\cite{Kolotouros_2019_ICCV}.} %\Note{SC: Add additional column to the  table. Still feel confusing.}
\label{tbl:quan_eval_multidata}
\end{table*}

\begin{table*}[thb!]
\centering
\tiny
\begin{tabular}{l | l | c | c | c | c | c | c | c | c | c | c | c | c | c | c }
  \hline
   \multicolumn{2}{l|}{} & \multicolumn{4}{|c|}{H36M P1} & \multicolumn{4}{|c|}{H36M P2} & \multicolumn{2}{|c|}{UP-3D} & \multicolumn{4}{|c}{LSP} \\
  \hline
     \multirow{2}{*}{No.} & \multirow{2}{*}{Methods} & MPJPE & RE & MPJPE & RE & MPJPE & RE & MPJPE & RE & Sh. Err. & Sh. Err. & \multirow{2}{*}{FB Acc.} & \multirow{2}{*}{FB F1} & \multirow{2}{*}{Parts Acc.} & \multirow{2}{*}{Parts F1} \\
     & & (np) & (np) & (p) & (p) & (np) & (np) & (p) & (p) & (np) & (p) & & & & \\
  \hline
     %A & G-CMR~\cite{kolotouros2019cmr} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3  & 71.9 & 50.1 & - & - & 91.46 & 88.6 9& 0.87 & 0.66  \\
     A & G-CMR~\cite{kolotouros2019cmr} & 73.99 & 54.87 & 77.52 & 57.78 & 73.52 & 53.97 & 75.61 & 56.13 & 104.49 & 122.93 & 90.52 & 0.85 & 87.90 & 0.64 \\
     B & G-CMR, 12 GRBs  & 83.19 & 56.56 & 85.19 & 58.17 & 80.69 & 54.44 & 82.91 & 56.15 & 110.5 & 112.2 & 90.64 & 0.85 & 87.89 & 0.64 \\

     C & G-CMR, 18 GRBs & 80.62 & 54.96 & 81.79 & 56.35 & 77.63 & 53.06  & 78.53 & 53.77 & 104.0 & 108.5 & 91.13 & 0.86 & 88.35 & 0.65 \\
     D & Pre W.share FL & 64.81 & 39.57 & 67.85 & 43.44 & 62.80 & 39.79  & 65.31 & 43.07  & 67.48 & 71.39 & 92.77 & \textbf{0.89} & 90.71 & 0.73 \\
     E & Pre No W.Share FL & \textbf{62.4} & \textbf{37.7} & \textbf{65.9} & 41.2 & \textbf{59.7} & \textbf{36.6} & 64.1 & 40.4 & \textbf{66.3} & \textbf{66.4} & \textbf{93.09} & \textbf{0.89} & \textbf{90.90} & \textbf{0.74} \\
     F & Post W.Share & 66.12 & 40.64 & 66.64 & 42.69 & 63.75 & 39.35 & 63.83 & 42.09 & 68.47 & 67.35 & 92.89 & \textbf{0.89} & 90.71 & 0.73\\
     G & Post No W.Share FL & 66.56 & 39.95 & 69.07 & 42.52 & 64.34 & 39.56 & 67.36 & 42.03 & 68.43 & 67.79 & 93.00 & \textbf{0.89} & 90.08 & 0.73 \\
     H & Pre W.Share & 72.36 & 42.45 & 79.36 & 49.25 &73.54& 43.41& 80.70 &48.90 & 84.24 & 79.52 & 92.06 & 0.88 & 89.84 & 0.70 \\
     I &  LeakyReLU & 63.30 & 39.09 & 64.64 & \textbf{41.08} & 61.72 & 38.71 & \textbf{62.52} & \textbf{40.13} & 71.80 & 68.78 & 92.54 & 0.88 & 90.41 & 0.72 \\
     J & Global Feat & 91.80 & 60.03 & 93.55 & 62.34 & 90.23 & 57.95 & 93.01 & 60.82 & 115.56 & 115.17 & 90.67 & 0.85 & 88.00 & 0.64 \\
     K & Non-Local (False) & 68.65 & 42.21 & 72.71 & 48.34 & 67.41 & 42.31 & 71.37 & 47.74 & 79.66 & 80.56 & 91.49 & 0.86 & 89.43 & 0.68 \\
     L & Non-Local (True) & 72.52 & 45.36 & 69.87 & 46.56 & 70.82 & 45.58 & 67.70 & 46.04 & 72.21 & 68.35 & 91.88 & 0.87 & 89.86 & 0.70 \\
  \hline
\end{tabular}
\caption{Evaluation results for ablation studies. \Note{SC: font size is too small.}}
\label{tbl:ablation_results}
\end{table*}

\subsection{Implementation}

The perceptual features which we compute for the branches, initially have different dimension between the mesh and joint branch, since they are assembled differently from the ResNet50 model. We first pass each through a graph linear to make the feature dimensions between both branches the same. This enables us to use weight sharing between the GRBs in the mesh and joint branch.

\subsection{Training details}
\label{subsec:training}
We use a pre-trained ResNet-50 for extracting perceptual features. Our model is trained end-to-end with a batchsize of 64 and learning rate of \(3e^{-4}\). Mini-batches during training are assembled by selecting images from the five training datasets. The composition is 30\%, 20\%, 10\%, 20\% and 20\% for Human 3.6M, UP-3D, LSP, COCO and MPII respectively. We shuffle the images in each dataset before random selection into mini-batches. Due to the difference in cardinality between the datasets, the training images for some datasets are used multiple times. The Adam optimizer is used to determine the weight updates. We train our model for fifty epochs, however we observed that fewer epochs yield almost the same result (see Section~\ref{subsec:ablation_studies} for more discussion). The regression of camera parameters in the mesh branch contains a graph linear layer, followed by a ReLU and a fully connected layer to produce three parameters for a weak perspective camera model. We found that this could lead to training instability. In particular, the weights for the fully connected layer can go to all zeros, in which case only the bias term determines the camera parameters. The ReLU prior to the fully connected layer can produce many zero values as output, eventually causing the weights to go to zero. To avoid this problem, we have tried different approaches: use leaky ReLU, insert InstanceNorm~\cite{DBLP:journals/corr/UlyanovVL16} and BatchNorm~\cite{Ioffe:2015:ICML} prior to the ReLU.

\subsection{Comparison with State-of-the-Art Methods}

\paragraph{Quantitative Evaluation}
We evaluate our model on the evaluation data mentioned earlier, and compare the results to several recent methods. We report our best performing configuration which uses weight sharing between the mesh and joint branch, pre-fusion, and focal loss applied to the 3D joint loss in the mesh branch, with parameters \(A=1\), \(B=5\) and \(\gamma=1\). The results are summarized in Table~\ref{tbl:quan_eval_multidata}. For Graph CMR~\cite{kolotouros2019cmr} we report two sets of numbers. The first are taken directly from the paper. However, we could not validate those numbers with the provided code and retrained their model from scratch using the training procedure from Section~\ref{subsec:training}. The numbers we obtain from retraining are listed in row A of Table 2.  \Note{SC: the metrics, such as MPJPE, RE, Sh. Err, in Table 1 are not explained.}

\paragraph{Qualitative Results}

Figure~\ref{fig:qualitative_results} shows several examples of successful reconstructions. In general the non-parametric result is a slightly better fit compared to the parametric result. The selected results are quite challenging due to multiple people or challenging poses. Figure~\ref{fig:failure_cases} shows two representative failure cases.
%The last XX rows illustrate the improvement over results obtained with Graph CMR~\cite{kolotouros2019cmr}. The second to last row compares our method to~\cite{Kolotouros_2019_ICCV}. Overall our reconstructions are a better fit. The final row in the figure shows some failure cases. Some poses remain challenging, and the performance is reduced in the presence of multiple people in an image.

\begin{figure*}[thb!]
    \centering
    \includegraphics[width=0.88\textwidth]{images/qualitative_result.pdf}
    \caption{Qualitative results. From left to right: input, non-parametric pose and shape, parametric pose and shape. Our method can recover accurate 3D shape and pose for challenging cases.}
    \label{fig:qualitative_results}
\end{figure*}

\begin{figure}[th!]
    \centering
    \includegraphics[width=\columnwidth]{images/failure_cases.pdf}
    \caption{Failure cases. Very challenging poses, occlusions, and multiple people lead to incorrect reconstructions. \Note{SC: explain left, middle, right.}}
    \label{fig:failure_cases}
\end{figure}

\subsection{Ablation Studies}
\label{subsec:ablation_studies}

% \begin{table}
% \centering
% \tiny
% \begin{tabular}{l | c | c | c | c | c || c | c }
%   \hline
%   & \multicolumn{2}{|c|}{H36M P1} & \multicolumn{2}{|c|}{H36M P2} & UP-3D & \multicolumn{2}{|c}{LSP} \\
%   \hline
%   \multirow{1}{*}{Methods} & \multirow{2}{*}{MPJPE} & \multirow{2}{*}{RE} & \multirow{2}{*}{MPJPE} & \multirow{2}{*}{RE} & \multirow{2}{*}{Sh. Err.} & FB Acc. & Parts Acc. \\
%      & & & & & & FB F1 & Parts F1 \\
% %  \hline
% %    Methods & \multicolumn{7}{c}{} \\
%   \hline
%      share + pre_fuse& 75.0 & 51.2 & 72.7 & 49.3 & - & 91.46 & 88.69 \\
%      share + post_fuse & 74.7 & 51.9 & 71.9 & 50.1 & - & 0.87 & 0.66 \\
%     \hdashline
%      not share + pre_fuse & 74.0 & 54.9 & 73.5 & 54.0 & 152.6 & 90.52 & 87.90 \\
%     18 GRBs & 77.5 & 57.6 & 75.6 & 56.1 & 200.3 & 0.85 & 0.65 \\
%     \hdashline
%     not share + post_fuse& - & - & - & - & - & 91.83 & 89.41 \\
%     Post-fusion & - & - & - & 41.1 & - & 0.87 & 0.68 \\
%     \hdashline
%     Ours & - & - & - & - & - & 91.83 & 89.41 \\
%     No W.Share & - & - & - & 41.1 & - & 0.87 & 0.68 \\
%     \hdashline
%     Ours & \textbf{62.4} & \textbf{37.7} & \textbf{59.7} & \textbf{36.6} & \textbf{66.3} & \textbf{93.09} & \textbf{90.90} \\
%     baseline & 65.9 & 41.2 & 64.1 & 40.4 & 66.4 & \textbf{0.89} & \textbf{0.74} \\
%   \hline
% \end{tabular}
% \vspace{5pt}
% \caption{Placeholder table to show we are awesome}
% \label{tbl:ablation_results}
% \end{table}

% \begin{table*}
% \centering
% \tiny
% \begin{tabular}{l | l | c | c | c | c | c | c | c | c | c | c | c | c | c | c }
%   \hline
%   \multicolumn{2}{l|}{} & \multicolumn{4}{|c|}{H36M P1} & \multicolumn{4}{|c|}{H36M P2} & \multicolumn{2}{|c|}{UP-3D} & \multicolumn{4}{|c}{LSP} \\
%   \hline
%      \multirow{2}{*}{No.} & \multirow{2}{*}{Methods} & MPJPE & RE & MPJPE & RE & MPJPE & RE & MPJPE & RE & Sh. Err. & Sh. Err. & \multirow{2}{*}{FB Acc.} & \multirow{2}{*}{FB F1} & \multirow{2}{*}{Parts Acc.} & \multirow{2}{*}{Parts F1} \\
%      & & (np) & (np) & (p) & (p) & (np) & (np) & (p) & (p) & (np) & (p) & & & & \\
%   \hline
%      %A & G-CMR~\cite{kolotouros2019cmr} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3  & 71.9 & 50.1 & - & - & 91.46 & 88.6 9& 0.87 & 0.66  \\
%      B & G-CMR~\cite{kolotouros2019cmr} & 73.99 & 54.87 & 77.52 & 57.78 & 73.52 & 53.97 & 75.61 & 56.13 & 104.49 & 122.93 & 90.52 & 0.85 & 87.90 & 0.64 \\
%      C & G-CMR, 12 GRBs  & 83.19 & 56.56 & 85.19 & 58.17 & 80.69 & 54.44 & 82.91 & 56.15 & 110.5 & 112.2 & 90.64 & 0.85 & 87.89 & 0.64 \\

%      D & G-CMR, 18 GRBs & 80.62 & 54.96 & 81.79 & 56.35 & 77.63 & 53.06  & 78.53 & 53.77 & 104.0 & 108.5 & 91.13 & 0.86 & 88.35 & 0.65 \\
%      E & Pre W.share FL & 64.81 & 39.57 & 67.85 & 43.44 & 62.80 & 39.79  & 65.31 & 43.07  & 67.48 & 71.39 & 92.77 & \textbf{0.89} & 90.71 & 0.73 \\
%      F & Pre No W.Share FL & \textbf{62.4} & \textbf{37.7} & \textbf{65.9} & 41.2 & \textbf{59.7} & \textbf{36.6} & 64.1 & 40.4 & \textbf{66.3} & \textbf{66.4} & \textbf{93.09} & \textbf{0.89} & \textbf{90.90} & \textbf{0.74} \\
%      G & Post W.Share & 66.12 & 40.64 & 66.64 & 42.69 & 63.75 & 39.35 & 63.83 & 42.09 & 68.47 & 67.35 & 92.89 & \textbf{0.89} & 90.71 & 0.73\\
%      H & Post No W.Share FL & 66.56 & 39.95 & 69.07 & 42.52 & 64.34 & 39.56 & 67.36 & 42.03 & 68.43 & 67.79 & 93.00 & \textbf{0.89} & 90.08 & 0.73 \\
%      I & Pre W.Share & 72.36 & 42.45 & 79.36 & 49.25 &73.54& 43.41& 80.70 &48.90 & 84.24 & 79.52 & 92.06 & 0.88 & 89.84 & 0.70 \\
%      J &  LeakyReLU & 63.30 & 39.09 & 64.64 & \textbf{41.08} & 61.72 & 38.71 & \textbf{62.52} & \textbf{40.13} & 71.80 & 68.78 & 92.54 & 0.88 & 90.41 & 0.72 \\
%      K & Global Feat & 91.80 & 60.03 & 93.55 & 62.34 & 90.23 & 57.95 & 93.01 & 60.82 & 115.56 & 115.17 & 90.67 & 0.85 & 88.00 & 0.64 \\
%   \hline
% \end{tabular}
% \vspace{5pt}
% \caption{Evaluation results for ablation studies.}
% \label{tbl:ablation_results}
% \end{table*}

In this section we evaluate various components and parameters of our proposed method.

\noindent \textbf{Study 1} \Note{SC: give a more specific name here?} Given that our model has an additional branch to predict joints, we train the model from~\cite{kolotouros2019cmr} with additional graph residual blocks. We have added 6 and 12 additional GRBs after its original backbone, and thus the model sizes are roughly equal to our GCN model with and without weight sharing. To make the training stable, we also apply the BatchNorm before the last ReLU of camera layers and train with focal loss on the 3D joints loss. Rows B and C in Table~\ref{tbl:ablation_results} show that our multi-scale approach outperforms both deeper models. \\
\textbf{Study 2} As discussed in Section~\ref{subsec:graph_fusion_blocks} we identify two fusion regimes: Pre- and Post-fusion. We have trained models with both regimes. From rows D-G in Table~\ref{tbl:ablation_results} we can see that Pre-fusion generally outperforms Post-fusion.\\
\textbf{Study 3} Given the definition of graph convolutions, when the feature dimensions for the nodes in the graph in both the mesh and joint branch are the same, the weights for the graph convolutions can be shared among the two branches and reduce the number of learnable parameters. We have trained models with and without weight sharing. From Table~\ref{tbl:ablation_results} we see that double the parameter size only gives a marginal performance gain (comapre rows D and F to E and G).  \\
\textbf{Study 4} We explore both global and local perceptual features to feed into the joint branch. The perceptual features attached to the nodes in the joint branch are computed from local regions around each 2D joint location in the images. We have trained a model which uses global perceptual features, like the mesh branch, instead. For a fair comparison, we keep the same GCN backbone as row E and use the global feature instead in row J. We can see that the model performance dramatically drops without the more descriptive local perceptual features. \\
\textbf{Study 5} All the experiments annotated with FL in ~\ref{tbl:ablation_results} apply the focal loss with \(A=1\) , \(B=5\) and \(\gamma = 1\). We have explored values for \(B\) in the range 5 to 10 and the performances are roughly the same. To determine the influence of the focal loss to the performance, we train our models with focal loss where \(B = 5\) and without focal loss. Compare rows D and H. Table~\ref{tbl:ablation_results} shows that the focal loss can help boost performance. As a regression task with dense prediction, the focal loss will more substantially penalize joints or vertices with large loss. The small ratio of bad predictions will not be ignored even if most predictions are good. It further improves the performance of our multi-scale architecture.\\
\textbf{Study 6} Since the nodes of the joint branch have full connection with the mesh nodes, they propagate information faster and provide non-local feature information to the mesh nodes. We would like to test whether Non-Local layers~\cite{Wang_2018} can further boost performance. We apply a Non-Local layer after each GRB in the joint branch using Pre-fusion, and with and without weight sharing. Rows K and L in Table~\ref{tbl:ablation_results} show the results. Surprisingly, non-local features reduce the performance when we already have a high-level graph structure. \\
\textbf{Study 7} We also explore some methods to solve the instability problem caused by the last ReLU in the prediction of camera parameters (see Sec.~\ref{subsec:training}). Both Replacing it with LeakyReLU and applying BatchNorm instead works well. In Table~\ref{tbl:ablation_results} all the experiments use BatchNorm, except for row I which uses LeakyReLU.

% \begin{figure}[th!]
%     \centering
%     \includegraphics[width=\columnwidth]{images/failure_cases.pdf}
%     \caption{Failure cases. Very challenging poses, occlusions, and multiple people lead to incorrect reconstructions.}
%     \label{fig:failure_cases}
% \end{figure}

%The idea from Non-Local Neural Networks~\cite{Wang_2018} can be exploited in our case as well. Efficient propagation of information from far away nodes in the graph instead of fusion blocks. 

% \begin{table}
% \centering
% \begin{tabular}{l|c|c}
%   \hline
%     Methods & Reconstr. & Acc.  \\
%   \hline
%     Graph CMR~\cite{} & 81.0 & 0.86 \\
%     Model fitting~\cite{} & 88.0 & 0.88 \\
%     Ours & 91.0 & 0.89 \\
%   \hline
% \end{tabular}
% \vspace{5pt}
% \caption{Placeholder}
% \label{tbl:deeper_graph_cmr}
% \end{table}

% \begin{table}[thb!]
% \centering
% \begin{tabular}{l|c|c}
%   \hline
%     Methods & Reconstr. & Acc.  \\
%   \hline
%     Graph CMR~\cite{} & 81.0 & 0.86 \\
%     Model fitting~\cite{} & 88.0 & 0.88 \\
%     Ours & 91.0 & 0.89 \\
%   \hline
% \end{tabular}
% \vspace{5pt}
% \caption{Placeholder}
% \label{tbl:focal_loss_compare}
% \end{table}

% \subsection{Additional Results} 
% \Note{SC: do we need this? Put this into Appendix?}


==> sections/tabels_backup.tex <==
\begin{comment}
\begin{table*}%[htb!]
\centering
\small
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline
 & \multicolumn{4}{c|}{H36M P1} & \multicolumn{4}{c|}{H36M P2} & \multicolumn{2}{c|}{UP-3D} & \multicolumn{4}{c}{LSP} \\ 
\hline
\multirow{2}{*}{Methods} & \tiny{MPJPE} & RE & \tiny{MPJPE}  & RE & \tiny{MPJPE}  & RE & \tiny{MPJPE}  & RE & \begin{tabular}[c]{@{}c@{}}Sh. \\Err. \end{tabular} & \begin{tabular}[c]{@{}c@{}}Sh. \\Err. \end{tabular} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB \\Acc. \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB\\F1 \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts\\Acc. \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts\\F1 \end{tabular}} \\
 & (np) & (np) & (p) & (p) & (np) & (np) & (p) & (p) & (np) & (p) & & & & \\ 
\hline
SMPLify~\cite{bogo2016keep} & - & - & - & - & - & - & - & 82.3 & - & - & - & - & - & - \\ 
Lassner~\cite{Lassner:UP:2017} & - & - & - & - & - & - & - & 93.9 & - & - & - & - & - & - \\ 
HMR~\cite{hmrKanazawa17} & - & - & 88.0 & 58.1 & - & - & - & 56.8 & - & - & 91.67 & 0.87 & 87.12 & 0.60 \\ 
NBF~\cite{omran2018neural} & - & - & - & - & - & - & - & 59.5 & - & - & - & - & - & - \\ 
Pavlakos~\cite{pavlakos2018learning} & - & - & - & - & - & - & - & 75.9 & - & - & - & - & - & - \\ 
Kanazawa~\cite{Kanazawa_2019_CVPR} & - & - & - & - & - & - & - & 56.9 & - & - & - & - & - & - \\ 
Arnab~\cite{arnab2019exploiting} & - & - & - & - & - & - & 77.8 & 54.3 & - & - & - & - & - & - \\ 
SPIN~\cite{Kolotouros_2019_ICCV} & - & - & - & - & - & - & - & 41.1 & - & - & 91.83 & 0.87 & 89.41 & 0.68 \\ 
I2L-MeshNet~\cite{moon2020i2l} & - & - & - & - & \textbf{55.7} & 41.1 & - & -  & - & - & - & - & - & - \\ 
\hline
%\begin{tabular}[c]{@{}l@{}}G-CMR\\~\cite{kolotouros2019cmr}\end{tabular} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3 & 71.9 & 50.1 & - & - & 91.46 & 0.87 & 88.69 & 0.66 \\
GraphCMR~\cite{kolotouros2019cmr} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3 & 71.9 & 50.1 & 104.5* & 122.9* & 91.46 & 0.87 & 88.69 & 0.66 \\
%\begin{tabular}[c]{@{}l@{}}G-CMR\\(same datasets)\end{tabular} & 74.0 & 54.9 & 77.5 & 57.8 & 73.5 & 54.0 & 75.6 & 56.1 & 104.5 & 122.9 & 90.52 & 0.85 & 87.90 & 0.64 \\ 
\hline            
%\begin{tabular}[c]{@{}l@{}}MFL\\~\cite{Kolotouros_2019_ICCV}\end{tabular} & - & - & - & - & - & - & - & 41.1 & - & - & 91.83 & 0.87 & 89.41 & 0.68 \\ 
%Ours1 &72.75& 48.77& 71.63& 49.97& 68.08& 46.22& 66.77& 47.52& 96.31&  96.64& 91.91& 0.87& 89.44& 0.68 \\
%Ours + GT 2D pose & \textbf{60.5} & \textbf{36.1} & \textbf{66.6} & \textbf{40.7} & \textbf{57.3} & \textbf{34.4} & \textbf{62.5} & \textbf{39.0} & \textbf{60.8} & \textbf{64.7} & \textbf{93.21} & \textbf{0.89} & \textbf{91.01} & \textbf{0.74} \\
Ours & \textbf{61.2} & \textbf{35.4} & \textbf{65.4} & \textbf{39.1} & 58.5 & \textbf{34.0} & \textbf{62.2} & \textbf{38.6} & \textbf{59.0} & \textbf{61.1} & \textbf{93.15} & \textbf{0.89} & \textbf{90.96} & \textbf{0.73} \\
\hline
\end{tabular} 
%\vspace*{-5pt}
\caption{Comparison of the metrics between different methods on H36M, UP-3D and LSP for estimated 3D poses (MJPE, RE), mesh (Sh.Err.) and 2D projection (FB Acc., Parts F1) respectively (*\textemdash results obtained by our training of~\cite{kolotouros2019cmr}). %{\it G-CMR(same datasets)} is retrained with the datasets and procedure from ~\ref{subsec:training}.
}
\label{tbl:quan_eval_multidata}               
\end{table*} 
\end{comment}


\begin{table*}%[t!]
\centering
\small
\begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c} 
\hline
\multicolumn{2}{l|}{}  & \multicolumn{2}{c|}{H36M P1}     & \multicolumn{2}{c|}{H36M P2}     & \multicolumn{2}{c|}{UP-3D}      & \multicolumn{4}{c}{LSP}  \\ 
\hline
\multirow{2}{*}{No.} & \multirow{2}{*}{Methods} & RE & RE & RE & RE & Sh. Err.  & Sh. Err. & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB \\Acc.\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB\\~F1\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts \\Acc.\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts \\F1\end{tabular}}  \\
&  & (np) & (p) & (np) & (p) & (np) & (p)  & & & &  \\ 
\hline
% # 76.394422    50.91033563  75.77594666  51.27315953, 
% 73.99751866  48.84267873  73.38045653  48.90001025
% 100.71520282 100.3755832
% [[0.9161004  0.8672217 ]
%  [0.89155901 0.67724103]]
A& Ours + Scheduled Sampling &  35.4 & \textbf{39.1}  & 34.0  & \textbf{38.6} & \textbf{59.0} & \textbf{61.1} & 93.15 & \textbf{0.89} & 90.96 & 0.73 \\
B& Ours + HRNet 2D joints & \textbf{35.2} &  42.3 &  \textbf{33.6} & 41.5 & 60.9 & 67.1 & 93.10 & \textbf{0.89} & 90.96 & 0.73 \\
C& Ours + GT 2D joints & 53.7 & 53.1 & 49.3& 49.3 & 86.9 & 90.4 & 93.0 & \textbf{0.89} & 90.77 & 0.73 \\
D& Ours + GT 2D joints (train and test) & 36.1 &  40.7 &  34.4 & 39.0 & 60.8 & 64.7 & \textbf{93.21} & \textbf{0.89} & 91.01 & \textbf{0.74} \\
\hline
E & no-GFB  & 50.9 &  51.3& 48.8 & 48.9 & 100.7 & 100.4 & 91.61 & 0.87 & 89.16 & 0.68 \\
%62.05, 36.74, 64.99, 40.01
F & GFB-as-first & 38.6  & 41.6 &  36.7 & 40.0 & 64.3  & 64.6 & 93.01 & \textbf{0.89} & 90.92 & 0.73\\
G & GFB-as-last & 38.7 & 40.9 &   38.3 &39.7 & 71.3 &70.9 & 92.52& 0.88 &90.21 &0.71\\
H & avgpool-as-fusion & 47.7 & 47.0 & 47.3 & 45.7 & 81.1 & 80.7 & 91.7&0.87 &89.20 &0.68 \\
I& maxpool-as-fusion & 43.8 & 43.6 & 42.9  & 42.9 & 77.0&  75.0& 91.8&0.87 &90.20 &0.70\\ \hline
%J & Skeleton-GCN without loss& 37.2 &  41.7&36.0  &39.8  &63.9 &  62.2 &  93.04& 0.89 & 90.90 &0.73\\ 
%K & Skeleton-GCN with gFeat & 48.8 & 50.0 & 46.2 & 47.5 & 96.3 & 96.6 & 91.9 & 0.87 & 89.44 & 0.68 \\ \hline
J & shared weight & 35.8 & 39.9 & 34.2 & 38.8 & 61.7 & 62.7 & 93.06 & \textbf{0.89} & 90.92 & 0.73 \\
K & no FL & 36.3 & 39.8 & 34.7 & 39.5 & 59.8 & 62.1 & 93.13 & \textbf{0.89} & \textbf{91.03} &  0.73 \\\hline
%L & fixed $\mathbf{A}_f$  & 37.7 & 41.2 & 36.6 & 40.4 & 66.3 & 66.4 & 93.09 & \textbf{0.89} & 90.90 & \textbf{0.74} \\
%M & fixed $\mathbf{A}_f$ + shared weight & 39.6 & 43.4 & 39.8 & 43.1 & 67.5 & 71.4 & 92.77 & \textbf{0.89} & 90.71 & 0.73 \\
%N & fixed $\mathbf{A}_f$ + shared weight + no FL & 42.5 & 49.3 & 43.4 & 48.9 & 84.2 & 79.5 & 92.06 & 0.88 & 89.84 & 0.70 \\

%I & Post W.Share, no FL & 40.64 & 42.69 & 39.35 & 42.09 & 68.47 & 67.35 & 92.89 & \textbf{0.89} & 90.71 & 0.73 \\
%J & Post & 39.95 & 42.52 & 39.56 & 42.03 & 68.43 & 67.79 & 93.00 & \textbf{0.89} & 90.08 & 0.73 \\\hline
%J & Global Feat & 60.03 & 62.34 & 57.95 & 60.82 & 115.56 & 115.17 & 90.67 & 0.85 & 88.00 & 0.64 \\
%M & Non-Local (False) & 42.21 & 48.34 & 42.31 & 47.74 & 79.66 & 80.56 & 91.49 & 0.86 & 89.43 & 0.68 \\
%N & Non-Local (True) & 45.36 & 46.56 & 45.58 & 46.04 & 72.21 & 68.35 & 91.88 & 0.87 & 89.86 & 0.70 \\ \hline
%J & gFeat FL & 60.03 & 62.34 & 57.95 & 60.82 & 115.56 & 115.17 & 90.67 & 0.85 & 88.00 & 0.64 \\
%N & gFeat BN & 52.27 & 53.51 & 49.36 & 50.85 & 99.90 & 101.25 & 91.60 & 0.87 & 89.18 & 0.68 \\
%K & B=10 & 39.02 & 42.35 & 38.05 & 41.37 & 71.74 & 71.86 & 92.25 & 0.88 & 90.16 & 0.71 \\ \hline
%P & B=10(True) & 43.09 & 46.97 & 43.23 & 45.76 & 89.21 & 86.34 & 92.30 & 0.88 & 90.15 & 0.71  \\ \hline
%L & LeakyReLU & 39.09 & \textbf{41.08} & 38.71 & \textbf{40.13} & 71.80 & 68.78 & 92.54 & 0.88 & 90.41 & 0.72 \\
%\hline
%M & G-CMR, 12 GRBs & 56.56 & 58.17 & 54.44 & 56.15 & 110.5 & 112.2 & 90.64 & 0.85 & 87.89 & 0.64 \\
%N & G-CMR, 18 GRBs & 54.96 & 56.35 & 53.06 & 53.77 & 104.0 & 108.5 & 91.13 & 0.86 & 88.35 & 0.65 \\ \hline
\end{tabular}
\caption{Evaluation results for ablation studies. See text for details. 
%We remove certain configuration from our best one as describe in Table~\ref{tbl:quan_eval_multidata} to learn the efficiency of each single proposed idea. Row E-I: we applied fixed adjacent matrix for fusion blocks. Row M-N: we use deeper GCN in Graph CMR~\cite{Kocabas_2019_CVPR}. FL is for focal loss, gFeat represents global feature, LeakyReLU is used instead of the last ReLU in camera layers, W.Share indicates the model shares weights between joint branch and mesh branch, No Adaptive A means we fixed the adjacent matrix of the fusion blocks, B is the parameter in Focal Loss.
}
\label{tbl:ablation_results_old}
\end{table*}


\begin{comment}

\begin{figure}[t!]
%\vspace{-10pt}
\centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_left_wrist.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_left_elbow.pdf} 
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_left_shoulder.pdf}
        \label{fig:subim11}
    \end{subfigure}
    \hspace{8pt}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\linewidth]{images/loss_kp_3d_fixed.png}%
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_right_pelvis.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_right_knee.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=0.95\linewidth]{images/joint2mesh/vis_adjmat_right_ankle.pdf}
        \label{fig:subim21}
    \end{subfigure}
    \hspace{8pt}
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\linewidth]{images/loss_shape_fixed.png}%
    \end{subfigure}    
\caption{(\textbf{columns 1-3}) A visualization of the learned adjacency matrix for GFBs. The weights for six joints are shown (clockwise, from top-left): left wrist, left elbow, left shoulder, right ankle, right knee, right pelvis. (\textbf{column 4}) Comparison of  \(\mathcal{L}_{kp3D}^M\)(left) and \(\mathcal{L}_{shape}^{M}\)(right) between the baseline (Orange) and our proposed model (Blue). We trained for 50 epochs and one epoch takes about 5,000 steps. Please note that we optimize Focal Loss instead of \(\mathcal{L}_{shape}^{M}\) when training the proposed model and we plot it here to compare with the baseline.}
\label{fig:visualize}
\end{figure}

\end{comment}

==> sections/table-eg.tex <==
    \begin{minipage}{.36\linewidth}
        \accuracyCompressionPlotWithLabels{0.46}{40}{61}{2.5pt}{data/cifar/cifar_2x100.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
        \vspace{-0.3cm}
        \subcaption{$2 \times 100$ @ CIFAR-10}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_2x200.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 200$ @ CIFAR-10}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_3x100.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $3 \times 100$ @ CIFAR-10}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}           
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_2x400.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 400$ @ CIFAR-10}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}            
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_4x100.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $4 \times 100$ @ CIFAR-10}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_2x800.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 800$ @ CIFAR-10}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{40}{61}{3.5pt}{data/cifar/cifar_5x100.txt}{0, 0.0001, 0.0002, 0.0003, 0.0004}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $5 \times 100$ @ CIFAR-10}
        \end{subfigure}
    \end{minipage}
    
    \vspace{0.4cm}
    
    \begin{minipage}{.36\linewidth}
        \accuracyCompressionPlotWithLabels{0.46}{18}{34}{2.5pt}{data/cifar_hundred/cifar_hundred_2x100.txt}{0,0.0002}
        \vspace{-0.3cm}
        \subcaption{$2 \times 100$ @ CIFAR-100}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_2x200.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 200$ @ CIFAR-100}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_3x100.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $3 \times 100$ @ CIFAR-100}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}           
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_2x400.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 400$ @ CIFAR-100}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}            
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_4x100.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $4 \times 100$ @ CIFAR-100}
        \end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{.2\linewidth}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_2x800.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize $2 \times 800$ @ CIFAR-100}
            \vspace{0.1cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \accuracyCompressionPlot{0.3}{18}{34}{3.5pt}{data/cifar_hundred/cifar_hundred_5x100.txt}{0,0.0002}
            \vspace{-0.1cm}
            \subcaption{\scriptsize  $5 \times 100$ @ CIFAR-100}
        \end{subfigure}
    \end{minipage}


    \caption{
    \textbf{{\color{bmblue}Test accuracy} and {\color{borange}nodes removed} for varying amounts of $\ell_1$ regularization.} The plots correspond to classifiers with different architectures on the (a)-(g) MNIST, %(h)-(n) CIFAR-10$^\text{G}$ (Gray) (o)-(u) CIFAR-10 (v)-(ab) CIFAR-100
    (h)-(n) CIFAR-10, and (o)-(u) CIFAR-100 datasets.  
    For each dataset, we keep the ranges of all the axes of the smaller plots  same as the bigger plot but hide the ticks for brevity.
    Networks trained with $\ell_1$ regularization can be exactly compressed, even when regularization improves accuracy. 
    }
    \label{fig:curves}
\end{figure}

==> sections/technical.tex <==
\section{Multi-Scale Graph Convolution Networks}
\label{sec:technical}

\begin{figure}[thb!]
    \centering
    \includegraphics[width=0.6\linewidth]{images/FusionBlockFig.pdf}
    \caption{The connection between the different graph scales can itself be considered a graph. A Graph Fusion Block (GFB) therefore has the same structure as a Graph Residual Block (GRB). \textbf{(a)} Pre-fusion: input from each branch to the fusion block is before the respective branches' GRBs.  \textbf{(b)} Post-fusion block: input from each branch to the fusion is after the branches' respective GRBs. Green boxes represent graph linear layers \Note{SC: what's graph linear layer?}, and red boxes represent graph convolutional layers.}
    \label{fig:graph_fusion_block}
\end{figure}



Figure~\ref{fig:architecture} shows the two branches of our network. The top branch is for predicting a 3D mesh, and is referred to as the mesh branch, or mesh GCN. The top branch has a similar architecture as~\cite{kolotouros2019cmr}. The bottom branch predicts the 3D joint locations of a skeleton. It also uses a GCN, and is denoted as the joint branch, or joint GCN. Each GCN branch consists of a number of graph residual blocks (GRB), the graph version of the bottleneck residual block~\cite{He2015DeepRL}. Each block consists of a graph linear layer, a group normalization~\cite{Wu_2018_ECCV}, a ReLU, graph convolution layer, another group normalization and ReLU and a final graph linear layer. The residual block has a skip connection, directly after the last graph linear layer. Information between the branches is exchanged via so-called fusion blocks, which are described in more detail in Section~\ref{subsec:graph_fusion_blocks}. In addition to a 3D mesh, the mesh branch also uses regression to produce three camera parameters of a weak perspective camera model. The camera model is used to project 3D joints onto the image to obtain 2D joints for supervision.

%The joint branch consists of GraphResBlock layers, and finally predicts a set of 3D joints. The mesh branch is similar to the Graph CMR network. The branches are trained simultaneously. The loss on 3D joints is  L2 loss (MSE loss). Using the regressed camera parameters from the mesh branch to project 3D joints onto the image, to determine the 2D joint loss.

\subsection{Image Feature Extraction}
The mesh branch attaches a global perceptual feature (obtained from ResNet-50 layers) to each vertex node of the template for the mesh GCN. In contrast, for the joint GCN we determine a more local perceptual feature to attach. Using the 2D joint location, we determine image region around the joint for which the feature is computed. If the input does not contain annotated 2D joint features, they can be estimated using methods such as~\cite{cao2017realtime, guler2018densepose, Habibie_2019_CVPR, Moon_2019_CVPR, Zhao_2019_CVPR, zhou_pami_2018}. We use the ROI Align from~\cite{he_mask_rcnn} to obtain the ROI over which the feature is computed. A few ROIs are denoted with red rectangles in the input image to the joint branch in Figure~\ref{fig:architecture}.

\subsection{Joint/Mesh Graph Convolution Networks} %\Note{SC: update it to the context of body joints and body meshes?}
Here we briefly state one layer in a graph convolution network; see details in~\cite{Kipf:2016tc}. Given a graph consisting of \(N\) nodes, and connectivity expressed by an adjacency matrix \(A\), the $l$th layer of graph convolution works as
\begin{align}
    X^{l+1} = f\left(\tilde{A}X^{l}W^{l}\right),
    \label{eq:graph_convolutions}
\end{align}
where \(\tilde{A}\) is the normalized adjacency matrix, \(X^{l}\) is the \(N \times D^{l}\) input to layer \(l\), and \(W^{l}\) is the \(D^{l} \times D^{l+1}\) weight matrix for layer \(l\). The activation function is denoted by \(f(.)\). We note that the weight matrix \(W^{l}\) operates on the features of the graph nodes, and does therefore not depend on the cardinality of the nodes in the graph. We will explain how we exploit this property for weight sharing below.  \Note{SC: refer to Figure 3?}

Note that~\eqref{eq:graph_convolutions} works for either the mesh scale or the joint scale by plugging a corresponding \(A\). For the mesh GCN, the graph topology is fully determined by the vertices and edges of the 3D mesh. For the joint GCN we define a graph with twelve nodes representing the 3D joints. The graph and its connections are depicted in the lower right corner of Figure~\ref{fig:architecture}.


\subsection{Adaptive Graph Fusion Block}
\label{subsec:graph_fusion_blocks}
As explained above, we want to exchange information between the two branches to inform the pose about the mesh detail, and vice versa. The ``connectivity" between joints and vertices can itself be considered a graph. The connectivity is likely determined in part by the proximity of joints to mesh vertices. However, the nodes may be connected, i.e., influenced, in additional, unknown, ways. We aim to learn this connectivity during training of our proposed model. We define Graph Fusion Blocks (GFB), depicted in Figures~\ref{fig:graph_fusion_block}(a) and (b), to exchange information between the branches. A GFB is implemeted as a GRB \Note{SC: what is GRB? J: Graph Residual Block, defined above.}. We propose an adaptive bipartite graph that describes the correspondence between joints and mesh nodes
Each element in the corresponding adjacency matrix \(A\) for the fusion layer is learnable during training. The normalization of \(A\) (see Eq.~\ref{eq:graph_convolutions}) in this case is done according to a Softmax. Finally, the weights for the fusion blocks are shared among all GFBs.

We distinguish two fusion approaches: pre-fusion and post-fusion. Pre-fusion, Fig.~\ref{fig:graph_fusion_block}(a), takes the input from the two branches before they are processed by each branches' GRB. Post-fusion on the other hand, takes the input after each branches' GRB, as shown in Figure~\ref{fig:graph_fusion_block}(b). Section~\ref{sec:experiments} provides a comparison of the fusion methods.

%Fusion blocks therefore employ the same graph residual block structure as those for the two branches of the network. We distinguish two fusion approaches: pre-fusion and post-fusion. Pre-fusion, depicted in Figure~\ref{fig:graph_fusion_block}(a), takes the input from the two branches before they are processed by each branches' graph residual block. Post-fusion on the other hand, takes input after each branches' graph residual block, as shown in Figure~\ref{fig:graph_fusion_block}(b). The expression of the connectivity between the joints and vertices as a graph requires adjacency information. The adjacency can be determined based on the proximity of joints and mesh vertices. We propose an adaptive adjacency, i.e., the elements in the adjacency matrix for the fusion layer are learned. We use the L2 distance between each joint and vertex as the initialization. The normalization of \(A\) (see Eq.~\ref{eq:graph_convolutions}) in this case is done using Softmax. Finally, the weights for the fusion blocks are shared among all fusion blocks.
%\Note{SC: details about the fusion block is missing. For example, how to merge the inputs from two branch, which have different shapes.}

Figure~\ref{fig:graph_fusion_matrix} shows the layout of the adjacency matrix. Given \(N_J\) nodes in the joint GCN, and \(N_V\) nodes in the mesh GCN, the full adjacency matrix would have a dimension of \((N_J + N_V) \times (N_J + N_V)\). For fusion we set the adjacency of the \((N_J \times N_J)\) and \((N_V \times N_V)\) sub-matrices to zero values. We thus only need to consider the two \(N_J \times N_V\) sub-matrices. \Note{SC: this paragraph is not necessary. this is a bipartite graph, mapping between the joints and the mesh nodes.} 

\begin{figure}[thb!]
    \centering
    \includegraphics[width=0.6\linewidth]{images/fusion_graph_matrix_fig.pdf}
    \caption{\textbf{(a)} The adjacency matrix used in the graph fusion blocks. Only the shaded parts contain non-zero elements. The dimensions are \((N_J + N_V) \times (N_J + N_V)\), where \(N_J\) is the number of joints, and \(N_V\) the number of vertices in the mesh.} % \textbf{(b)} Visualization of examples of the \((N_V \times N_J)\) and \((N_J \times N_V)^T\) learned weights.} 
    \label{fig:graph_fusion_matrix} \Note{SC: We only need to show the orange part, which is a bipartite graph. Label rows as joints and columns as mesh nodes.}
\end{figure}

The input to the graph from the joint branch is of dimension \(N_J \times F_1\), with \(F_1\) representing the features attached to the nodes. For the mesh branch the dimension is \(N_V \times F_2\). In the case where \(dim(F_1) \neq dim(F_2)\) we would need graph linear layers to make the dimensions equal prior to processing by the GRB. In this paper we only consider \(dim(F_1) = dim(F_2)\), which allows us to share weights between the two branches. After the fusion block, the output is of dimensions \(N_J \times F'_1\) and \(N_V \times F'_2\). Outputs are added to the respective branches, so the feature dimensions \(F'_1\) and \(F'_2\) are the same as that of \(F_1\) and \(F_2\).

%(but feature dimension can be different between branches, and we do not share weights between branches).
\subsection{Output}

The mesh GCN follows~\cite{kolotouros2019cmr} and outputs a set of deformed vertices of the template input mesh, together with the SMPL \( (\theta, \beta)\) parameters for pose and shape~\cite{SMPL:2015}. Using SMPL regression matrices, a set of 3D joints, which we label \emph{keypoints}, can be obtained for both the non-parametric mesh as well as the parametric SMPL result. The joint GCN outputs twelve predicted 3D joint locations.

\subsection{Loss function}
%\Note{SC: It lacks one overall loss function}
The loss from~\cite{kolotouros2019cmr} is extended with additional \(L_2\) loss terms. The losses are computed as MSE losses of the form:

\begin{align}
\nonumber
    \mathcal{L}_{MSE} = \frac{1}{N}\sum_{i=1}^{N} \left\|\hat{X} - X\right\|^2_2,
\end{align}
where \(\hat{X}\) is either the estimated 3D keypoint or joint, or the 2D keypoint or joint after projection. The combined loss function for training end-to-end is then:

\begin{equation} 
\nonumber \label{eq1}
\begin{split}
    \mathcal{L} = \hspace{3pt} &  \mathcal{L}_{shape} + \mathcal{L}_{kp2D} + \mathcal{L}_{kp3D} + \mathcal{L}_{\theta} + \mathcal{L}_{\beta} + \\
     & \mathcal{L}_{shape}^{smpl} + \mathcal{L}_{kp2D}^{smpl} + \mathcal{L}_{kp3D}^{smpl} + \mathcal{L}_{J2D} + \mathcal{L}_{J3D},
\end{split}
\end{equation}
{\HC where ... }\Note{SC: need to explain each term}

The authors in~\cite{2017FocalLF} propose a \emph{focal loss} with the intent of emphasizing hard to train examples in a classification task. We employ an analogous method for regression to penalize joints or vertices which have a relatively large distance (and thus larger loss) from the ground truth data, as this may lead to decreased overall performance. We also denote this as a focal loss, but our formulation has a different form:


\begin{align}
\nonumber
    \mathcal{L}_{fl} = -B (A \cdot \mathcal{L}_{L_1})^{\gamma} \log(1-A \cdot \mathcal{L}_{L_1}).
\end{align}


We apply this focal loss to the 3D or 2D keypoint or joint losses only. {\HC Note that in the case of using the focal loss, the initial penalty is an average \(L_1\) error rather than MSE.}\Note{SC: which terms are using focal loss? which terms are using L1 loss? which terms are using MSE loss?  }

==> sections/technical_cvpr21.tex <==
\section{Problem Formulation}
Our goal is to jointly estimate a 3D human pose and recover a complete 3D mesh based on a single input RGB image without knowing camera parameters. Mathematically, let $\mathbf{I} \in  \mathbb{R}^{H \times W \times 3}$ be an RGB image with the height $H$ and the width $W$, $\mathbf{V}_{\bf s} \in \mathbb{R}^{N_{\bf s} \times 3}$ be the 3D coordinates of $N_s$ body joints, indicating a 3D skeleton-based human pose, and $\mathbf{V}_{\bf m} \in \mathbb{R}^{N_{\bf m} \times d}$ be the 3D coordinates of $N_m$ mesh nodes, indicating a 3D mesh-based human shape. We aim to propose a model $\mathcal{F}(\cdot)$ so that $\widehat{\mathbf{V}}_{\bf s}, \widehat{\mathbf{V}}_{\bf m} = \mathcal{F}(\mathbf{I})$, where $\widehat{\mathbf{V}}_{\bf s}$ and $\widehat{\mathbf{V}}_{\bf m}$ are the estimated human pose and the recovered human mesh, which precisely approximate the targets $\mathbf{V}_{\bf s}, \mathbf{V}_{\bf m}$, respectively.

This joint task naturally requires to model a human body at two scales: a skeleton (coarser) scale and a mesh (finer) scale. To explicitly model the data correlations at two scales, we propose a~\emph{two-layer graph structure} that consists of a skeleton graph $G_s(\mathcal{V}_s, {\bf A}_s)$, a mesh graph $G_m(\mathcal{V}_m, {\bf A}_m)$ and a fusion graph $G_f(\mathcal{V}_s \cup {V}_m, {\bf A}_f)$. where $\mathcal{V}_s, \mathcal{V}_m$ are the node sets and ${\bf A}_s \in \mathcal{R}^{N_s \times N_s}, {\bf A}_m \in \mathcal{R}^{N_m \times N_m}, {\bf A}_f \in \mathcal{R}^{(N_m+N_s) \times (N_m+N_s)}$ are the corresponding graph adjacency matrices. $|\mathcal{V}_s| = N_s= 12$, reflecting $12$ body joints, and $|\mathcal{V}_m| = N_m = 1723$, reflecting $1723$ mesh nodes. 
The adjacency matrix of a fusion graph is ${\bf A}_f =  \begin{bmatrix} \bf{0} & {\bf A}_f^{s\rightarrow m}  \\ {\bf A}_f^{m \rightarrow s} & \bf{0} \end{bmatrix}$,  where ${\bf A}_f^{s\rightarrow m} \in \mathbb{R}^{N_s \times N_m}$ mapping body joints to mesh nodes, ${\bf A}_f^{m\rightarrow s} \in \mathbb{R}^{N_m \times N_s}$ mapping mesh nodes to body joints. Each one could be considered as a bipartite graph.

Note that ${\bf A}_s,{\bf A}_m$ are fixed and given based on the human body prior; see the predefined graph topology in the lower left corner of Figure~\ref{fig:architecture};  while ${\bf A}_f$ is data-adaptive during the training.

This two-layer graph structure is a core of the proposed system and brings two benefits: First, it naturally models a human body from both mesh and skeleton aspects, promoting feature extraction at two scales. Second, a fusion graph enables information exchange between two scales of a human body, mutually enhancing feature extraction at two scales and improving the performances in two tasks. 

\section{Two-Layer-graph Neural Network}
\label{sec:technical}
Based on the proposed two-layer graph structure, we design a graph neural network architecture to extract human body information from an RGB image and achieve 3D shape recovery and pose estimation at the same time. Figure~\ref{fig:architecture} shows the overall architecture, which consists of four modules: the image encoder module, the mesh graph module, the skeleton graph module and the fusion graph module. The mesh graph module (on the top) is to estimate a 3D mesh through a mesh graph neural network and the skeleton graph module (on the bottom) is to estimate the coordinates of 3D body joints through a skeleton graph neural network. The fusion graph module enables intermediate feature exchange across two above modules. Before we dive into each module, we first introduce image encoder module to extract image feature  as inputs of the graph modules, and a computational building block that will be used in both mesh and skeleton graph modules. 

\subsection{Image Encoder Module}
\label{subsec: feature_extraction}
The functionality of an image encoder module is to extract informative visual features from an RGB image, which would be the input for the subsequent modules. Mathematically, given an input RGB image $\mathbf{I}$,  $\{ \mathbf{X}^{(\ell)}_{\rm im} \}_{\ell=1}^{L} =  \mathcal{F}_{\rm im} \left( \mathbf{I} \right) \in \mathbb{R}^{H_{\ell} \times W_{\ell} \times D_{\ell}}$ is the output of the network, which is a collection of intermediate image features, where $H_{\ell}, W_{\ell}, D_{\ell}$ are the image height, width and channel number at the $\ell$-th convolution layer, and $\mathcal{F}_{\rm im}(\cdot)$ is a CNN whose architecture follows ResNet50~\cite{he2016deep}.

\subsection{Graph Residual Block} 
A graph residual block is an elementary computational unit for feature learning and propagation based on a graph structure. It consists of a sequence of a graph linear layer, a graph convolution layer, and another graph linear layer, with a residual connection from the input directly to the output of this block. Each layer follows a group normalization layer~\cite{Wu_2018_ECCV} and ReLU. To define a graph convolution layer, we use the skeleton graph as example, but the same procedure can be applied to the mesh graph. Let $\mathbf{X}_{\rm in} \in \mathbb{R}^{N_s \times d_{\rm in}}$ be the features of body joints. The output feature after the graph convolution layer is defined as
\begin{equation}
\label{eq:graph_convolutions}
    \mathbf{X}_{\rm out} = \sigma \left( {\bf A}_s \mathbf{X}_{\rm in}   \mathbf{W} \right) \in \mathbb{R}^{N_s \times d_{\rm out}},
\end{equation}
where ${\bf A}_s \in \mathbb{R}^{N_s \times N_s}$ is a graph adjacency matrix for a human skeleton, $\mathbf{W} \in \mathbb{R}^{d_{\rm in} \times d_{\rm out}}$ is a trainble weight matrix and $\sigma(\cdot)$ is an nonlinear activation function. The graph convolution layer~\eqref{eq:graph_convolutions} allows feature propagation over the skeleton graph so that each body joint can aggregate information from its neighbors. The graph linear layer simply substitutes the graph adjacency matrix $ {\bf A}_s$ in the graph convolution layer~\eqref{eq:graph_convolutions} to an identity matrix.

\subsection{Mesh Graph Module (Mesh-GCN)}
The functionality of a mesh graph module is to deform a template human mesh in neutral (T-)pose to a shaped and posed %high-quality %
3D  mesh conditioned on the input image features. Let $\mathbf{x}_{\rm global} = {\rm Pool_g}(\mathbf{X}^{(L)}_{\rm im}) \in \mathbb{R}^D$ be the global image feature with $ {\rm Pool_g}(\cdot)$ the global pooling operation and $\mathbf{V}^{(\rm neutral)}_m \in \mathbb{R}^{N_m \times 3}$ be the 3D coordinates of mesh nodes in a standardized neutral pose, whose $i$-th row, $\mathbf{v}_i \in \mathbb{R}^3$, are the 3D coordinates of the $i$-th mesh node. For each mesh node, we concatenate the global image features and the 3D coordinates, leading to an initialized mesh feature matrix $\mathbf{V}^{(0)}_m \in \mathbb{R}^{N_m \times (D+3)}$, with $i$-th row: $[\mathbf{v}_i; \mathbf{x}_{\rm global}] \in  \mathbb{R}^{D+3}$. The recovered 3D mesh is then $\widehat{\mathbf{V}}_m =  \mathcal{F}_{\rm m} \left( \mathbf{V}^{(0)}_m, {\bf A}_m \right) \in \mathbb{R}^{N_m \times 3}$, where ${\bf A}_m \in \mathbb{R}^{N_m \times N_m}$ is the mesh graph and $\mathcal{F}_{\rm m} (\cdot)$ is a graph neural network that consists of several stacked graph residual blocks. Intuitively, the graph neural network  implements the deforming process with the global image feature  $\mathbf{x}_{\rm global}$ as the deforming mechanism.

\subsection{Skeleton Graph Module (Skeleton-GCN)}
\label{susec:skeleton}
The functionality of a skeleton graph module is to lift the 2D pose estimated from an input RBG image to a 3D pose. Given the image, we use HRNet~\cite{sun2019deep} to estimate the 2D positions of body joints in this image. For each body joint, we crop a patch centered at the estimated 2D positions with the size of the average estimated bone length from the joints per image, using RoI Align~\cite{he_mask_rcnn} from the $\ell$-th image feature map $\mathbf{X}_{\rm image}^{(\ell)}$. This feature patch reflects the local visual information around the corresponding body joint. Mathematically, let $\mathbf{V}^{(0)}_s \in \mathbb{R}^{N_s \times d_f}$ be an initial skeleton feature matrix, where $d_f = \sum_{\ell=1}^L{{\overline H_{\ell}} {\overline W_{\ell}} {\overline D_{\ell}}} + 2$ and whose $i$-th row is $[\widehat{\mathbf{s}}_i;
{\rm \mathbf{RoI}(\mathbf{X}_{\rm im}^{(1)}, \widehat{\mathbf{s}}_i)};\dots;{\rm \mathbf{RoI}(\mathbf{X}_{\rm im}^{(L)}, \widehat{\mathbf{s}}_i)}] \in \mathbb{R}^{d_f}$, where $\mathbf{RoI}(\cdot)$ returns an $\overline{H_{\ell}} \times \overline{W_{\ell}}$ image feature patch from $\mathbf{X}_{\rm im}^{(\ell)}$ using RoI align with the patch centered at the 2D position of the $i$-th body joint $\widehat{\mathbf{s}}_i \in \mathbb{R}^2$, estimated by HRNet.

The estimated 3D pose is then, $\widehat{\mathbf{V}}_s =  \mathcal{F}_{\rm s} \left( \mathbf{V}^{(0)}_s \right)$. Similar to the Mesh-GCN, $\mathcal{F}_{\rm s}(\cdot)$ is a graph neural network that consists of stacked graph residual blocks.

%\begin{figure}[thb!]
%    \centering
%    \includegraphics[width=0.5\linewidth]{images/feature_pool.pdf}
%    \caption{Joint feature: concatenate multi-scale image feature of the bounding box centered at the joint extracted from conv layer 1 to 4 in ResNet using RoI Align~\cite{he_mask_rcnn}. TDB: This is a figure placeholder, which will be updated later.}
%    \label{fig:graph_feature_pool}
%\end{figure}

\subsection{Fusion Graph Module (Fusion-GCN)}
\label{subsec:graph_fusion_blocks}
The functionality of a fusion graph module is to enable information exchange between the Skeleton-GCN and Mesh-GCN modules and mutually enhance both tasks of 3D shape recovery and pose estimation. The input of this module are the intermediate features from Skeleton-GCN and Mesh-GCN. This module fuses those intermediate features and populates them back to both Skeleton-GCN and Mesh-GCN.

To fuse features from two modalities, we leverage a trainable fusion graph $G(\mathcal{V}_s \cup {V}_m, {\bf A}_f)$, which reflects the connectivity between body joints and mesh nodes. Instead of defining any fixed connections, we allow the two bipartite graph structures ${\bf A}_f^{m \rightarrow s}$ and ${\bf A}_f^{s \rightarrow m}$ to be trainable to capture the connectivity in the hidden feature space in a data-driven manner. To obtain this graph, we first initialize the fusion graph by the Euclidean distance between a mesh node and a body joint  of the template in standardized neutral pose. We take ${\bf A}_f^{m \rightarrow s}$ as example, $\left( {\bf A}_f^{(0), m\rightarrow s} \right)_{i,j} = 1/d_{ij}$ where $d_{ij} $ is the Euclidean distance between the $i$-th mesh node and $j$-th body joint  at the neutral pose. We scale $(\mathbf{A}_f^{(0), m\rightarrow s})_{i,j}$ by a trainable factor $\mathbf{U}^{m \rightarrow s}_{i,j}$ to learn the edge weights between the body joints and mesh nodes adaptively from data. Therefore, the trainable graph is defined as $\mathbf{A}_f^{m \rightarrow s} = \mathbf{U}^{m \rightarrow s} \odot \mathbf{A}_f^{(0), m \rightarrow s}$, where $\mathbf{U}^{m \rightarrow s} \in \mathbb{R}^{N_m \times N_s}$ is a trainable edge weight matrix and $\odot$ denotes element-wise product. Similarly, let $\mathbf{A}_f^{s\rightarrow m} = \mathbf{U}^{s \rightarrow m} \odot {(\mathbf{A}_f^{(0), m\rightarrow s})}^\intercal$ denote the trainable graph mapping from skeleton to mesh,  where $\mathbf{U}^{s \rightarrow m} \in \mathbb{R}^{N_s \times N_m}$. We normalize $\mathbf{A}_f^{m\rightarrow s}$ and $\mathbf{A}_f^{s\rightarrow m}$ such that each row sums to 1.

%\Note{SC: do you have two trainable edge weight matrix?? XIN: Yes, the large bipartite graph 
%
%($ \mathbb{R}^{(N_s + N_m) \times (N_s + N_m)}$) consists of two non-zero blocks: $\mathbf{A}_f^{m \rightarrow s} \in \mathbf{R}^{N_m \times N_s}$ and $\mathbf{A}_f^{s \rightarrow m} \in \mathbf{R}^{N_s \times N_m}$, both of which are trainable.  JVB: removed Norm(.) but commented out, so can be put back if needed. XIN: we normalize each row of the edge weight matrix to make each row sum to 1. How to describe it correctly?}


Based on the trainable fusion graph ${\bf A}_f^{s\rightarrow m}$ and ${\mathbf{A}_f^{m\rightarrow s}}$, the graph fusion block collects features from both Mesh-GCN and Skeleton-GCN and distributes the updated features back to the other module; illustrated in Figure~\ref{fig:graph_fusion_block}. This information propagation involves a skeleton graph block, a fusion graph block and a mesh graph block and is denoted as a graph fusion block (GFB). 

Let $\mathbf{V}^{(\ell)}_m \in \mathbb{R}^{N_m \times d_{\ell}}$ be the mesh feature matrix in the $\ell$-th mesh graph layer and
$\mathbf{V}^{(\ell)}_s \in \mathbb{R}^{N_s \times d_{\ell}}$ be the skeleton feature in the $\ell$-th skeleton graph layer. The fusion graph module will update the features as $\mathcal{V}_f^{(\ell),s \rightarrow m} = \mathcal{F}_{\rm f}^{(\ell), s\rightarrow m}(\mathbf{V}_s^{(\ell)}, \mathbf{A}_f^{s\rightarrow m})$ for the mesh graph, $\mathcal{V}_f^{(\ell), m \rightarrow s} = \mathcal{F}_{\rm f}^{(\ell), m\rightarrow s}(\mathbf{V}_m^{(\ell)}, \mathbf{A}_f^{m\rightarrow s})$ for the skeleton graph, which will be added back to the 
output from the graph residual blocks in two corresponding graph modules, respectively.

\begin{figure}[t]
    \centering
    %\includegraphics[width=0.8\linewidth]{images/FusionBlockFig4.pdf}
    \includegraphics[width=0.7\linewidth]{images/FusionBlock_Latest2.pdf}
    \caption{A Graph Fusion Block (GFB) consists of a Fusion-GCN block, a Mesh-GCN block and a Fusion-GCN block, each with the structure of the Graph Residual Block (GRB). The fusion block depicted here has its input from each branch prior to the GRBs, and adds its output back to each branch after their respective GRBs. Green boxes represent graph linear layers, dark red boxes represent graph convolutional layers.}
    \label{fig:graph_fusion_block}
\end{figure}
%The features are fed into a GFB block and updated as $\mathbf{V}_m^{(\ell+1)}= \mathcal{F}_{\rm m}^{(\ell)}(V_m^{(\ell)}, \mathbf{A}_m) + \mathcal{F}_{\rm f}^{(\ell), s\rightarrow m}(\mathbf{V}_s^{(\ell)}, \mathbf{A}_f^{s\rightarrow m})$ for the mesh graph and $\mathbf{V}_s^{(\ell+1)}= \mathcal{F}_{\rm s}^{(\ell)}(V_s^{(\ell)}, \mathbf{A}_s) + \mathcal{F}_{\rm f}^{(l), m\rightarrow s}(\mathbf{V}_s^{(\ell)}, \mathbf{A}_f^{m\rightarrow s})$ for the skeleton graph. 


%\subsection{Architecture Discussions}
%The Skeleton-GCN and Mesh-GCN extract features at two different scales of a human. We can consider a skeleton graph as a coarser graph representation of a mesh graph. Then, a two-layer graph is essentially a multi-scale representation of a mesh graph and makes information easier to propagate over the mesh graph.  Given the mesh graph only, the \textit{mesh-node}-to-\textit{mesh-node} connection is the only way to diffuse information between two mesh nodes. When two mesh nodes are far away from each other, it requires a large number of graph residual blocks to diffuse information between them. With the skeleton graph, there would be another path for two mesh nodes; i.e., a mesh node connects to a body joint, a body joint connects to another body joint, and finally, a body joint back to another mesh node. The  \textit{body-joint}-to-\textit{body-joint} connection is acting like a ``high-way'' to connect two mesh nodes, leading to more efficient information propagation. Experimentally, we observe that the skeleton graph helps speedup the convergence of mesh recovery; see Section~\ref{sec:experiments} for more discussion.

\subsection{Final estimation of human pose and mesh}
The Skeleton-GCN and Mesh-GCN output the estimated body joints $\widehat{\mathbf{V}}_s$ and the recovered mesh vertices $\widehat{\mathbf{V}}_m$ respectively. The mesh $\widehat{\mathbf{V}}_m$ is non-parametric, however, a parametric representation of the human body can be very useful for down-stream tasks (e.g., body manipulation). Similar to Graph CMR~\cite{kolotouros2019cmr}, given the predicted mesh $\widehat{\mathbf{V}}_m$, we train a MLP module to regress pose ($\widehat{\theta}$) and shape ($\widehat{\beta}$) parameters for a SMPL model~\cite{SMPL:2015}. To strengthen the consistency between the parametric and non-parametric representation of the body, and between the body mesh and 3D pose, we regress both the mesh and 3D pose from the estimated SMPL parameters ($\widehat{\theta}, \widehat{\beta}$) together with an additional 3D pose from $\widehat{\mathbf{V}}_m$ using the SMPL regression matrices~\cite{SMPL:2015}. Let $\widehat{\mathbf{V}}_m^{\rm smpl}, \widehat{\mathbf{V}}_s^{\rm smpl}$, $\widehat{\mathbf{V}}_s^{\rm mgcn}$ denote body mesh and 3D pose regressed from either the predicted SMPL or Mesh-GCN. We then define a mesh set as $\widehat{\mathbf{V}}_{\rm meshes} = \{\widehat{\mathbf{V}}_m, \widehat{\mathbf{V}}_m^{\rm smpl}\}$, and a 3D pose set as $\widehat{\mathbf{V}}_{\rm poses}^{3d}=\{\widehat{\mathbf{V}}_s, \widehat{\mathbf{V}}_s^{\rm smpl}, \widehat{\mathbf{V}}_s^{\rm mgcn}\}$.

To enable training on datasets which contain mostly 2D poses (e.g., COCO~\cite{MSCOCO_ECCV_2014}), a module consisting of graph layers predicts weak perspective camera parameters from the intermediate features of the Mesh-GCN (see ~\cite{kolotouros2019cmr} for the details). Using the weak perspective camera model, we can project the estimated 3D poses $\widehat{\mathbf{V}}_{\rm poses}^{3d}$ to obtain 2D poses, i.e., $\widehat{\mathbf{V}}_{\rm poses}^{2d}=\{\widehat{\mathbf{V}}_{s2d}^{\rm sgcn}, \widehat{\mathbf{V}}_{s2d}^{\rm smpl}, \widehat{\mathbf{V}}_{s2d}^{\rm mgcn}\}$, where ``$\rm sgcn$'' indicates regressed from the Skeleton-GCN. We next explain how we use this information for training.

\begin{table*}%[htb!]
\centering
\small
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c|c} 
\hline
 & \multicolumn{4}{c|}{H36M P1} & \multicolumn{4}{c|}{H36M P2} & \multicolumn{2}{c|}{UP-3D} & \multicolumn{4}{c}{LSP} \\ 
\hline
\multirow{2}{*}{Methods} & \tiny{MPJPE} & RE & \tiny{MPJPE}  & RE & \tiny{MPJPE}  & RE & \tiny{MPJPE}  & RE & \begin{tabular}[c]{@{}c@{}}Sh. \\Err. \end{tabular} & \begin{tabular}[c]{@{}c@{}}Sh. \\Err. \end{tabular} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB \\Acc. \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}FB\\F1 \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts\\Acc. \end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Parts\\F1 \end{tabular}} \\
 & (np) & (np) & (p) & (p) & (np) & (np) & (p) & (p) & (np) & (p) & & & & \\ 
\hline
SMPLify~\cite{bogo2016keep} & - & - & - & - & - & - & - & 82.3 & - & - & - & - & - & - \\ 
Lassner~\cite{Lassner:UP:2017} & - & - & - & - & - & - & - & 93.9 & - & - & - & - & - & - \\ 
HMR~\cite{hmrKanazawa17} & - & - & 88.0 & 58.1 & - & - & - & 56.8 & - & - & 91.67 & 0.87 & 87.12 & 0.60 \\ 
NBF~\cite{omran2018neural} & - & - & - & - & - & - & - & 59.5 & - & - & - & - & - & - \\ 
Pavlakos~\cite{pavlakos2018learning} & - & - & - & - & - & - & - & 75.9 & - & - & - & - & - & - \\ 
Kanazawa~\cite{Kanazawa_2019_CVPR} & - & - & - & - & - & - & - & 56.9 & - & - & - & - & - & - \\ 
Arnab~\cite{arnab2019exploiting} & - & - & - & - & - & - & 77.8 & 54.3 & - & - & - & - & - & - \\ 
SPIN~\cite{Kolotouros_2019_ICCV} & - & - & - & - & - & - & - & 41.1 & - & - & 91.83 & 0.87 & 89.41 & 0.68 \\ 
I2L-MeshNet~\cite{moon2020i2l} & - & - & - & - & \textbf{55.7} & 41.1 & - & -  & - & - & - & - & - & - \\ 
\hline
%\begin{tabular}[c]{@{}l@{}}G-CMR\\~\cite{kolotouros2019cmr}\end{tabular} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3 & 71.9 & 50.1 & - & - & 91.46 & 0.87 & 88.69 & 0.66 \\
GraphCMR~\cite{kolotouros2019cmr} & 75.0 & 51.2 & 74.7 & 51.9 & 72.7 & 49.3 & 71.9 & 50.1 & 104.5* & 122.9* & 91.46 & 0.87 & 88.69 & 0.66 \\
%\begin{tabular}[c]{@{}l@{}}G-CMR\\(same datasets)\end{tabular} & 74.0 & 54.9 & 77.5 & 57.8 & 73.5 & 54.0 & 75.6 & 56.1 & 104.5 & 122.9 & 90.52 & 0.85 & 87.90 & 0.64 \\ 
\hline            
%\begin{tabular}[c]{@{}l@{}}MFL\\~\cite{Kolotouros_2019_ICCV}\end{tabular} & - & - & - & - & - & - & - & 41.1 & - & - & 91.83 & 0.87 & 89.41 & 0.68 \\ 
%Ours1 &72.75& 48.77& 71.63& 49.97& 68.08& 46.22& 66.77& 47.52& 96.31&  96.64& 91.91& 0.87& 89.44& 0.68 \\
%Ours + GT 2D pose & \textbf{60.5} & \textbf{36.1} & \textbf{66.6} & \textbf{40.7} & \textbf{57.3} & \textbf{34.4} & \textbf{62.5} & \textbf{39.0} & \textbf{60.8} & \textbf{64.7} & \textbf{93.21} & \textbf{0.89} & \textbf{91.01} & \textbf{0.74} \\
Ours & \textbf{61.2} & \textbf{35.4} & \textbf{65.4} & \textbf{39.1} & 58.5 & \textbf{34.0} & \textbf{62.2} & \textbf{38.6} & \textbf{59.0} & \textbf{61.1} & \textbf{93.15} & \textbf{0.89} & \textbf{90.96} & \textbf{0.73} \\
\hline
\end{tabular} 
%\vspace*{-5pt}
\caption{Comparison of the metrics between different methods on H36M, UP-3D and LSP for estimated 3D poses (MJPE, RE), mesh (Sh.Err.) and 2D projection (FB Acc., Parts F1) respectively (*\textemdash results obtained by our training of~\cite{kolotouros2019cmr}). %{\it G-CMR(same datasets)} is retrained with the datasets and procedure from ~\ref{subsec:training}.
}
\label{tbl:quan_eval_multidata}               
\end{table*} 

\section{Training Strategy}
Here we introduce the loss function and scheduled sampling during training.
\label{sec:training}
%similarly, {\it Skeleton-GCN} indicates being regressed from Skeleton-GCN model and {\it s2d} indicates 2D pose.

%{\HC
%As the parametric representation of the human body is very useful for the down-stream tasks (e.g., body manipulation), we follow Graph CMR~\cite{kolotouros2019cmr} and train a MLP module to regress pose ($\widehat{\theta}$) and shape ($\widehat{\beta}$) parameters for a SMPL model~\cite{SMPL:2015} given the predicted mesh $\widehat{\mathbf{V}}_m$. To strengthen the consistency between the parametric and non-parametric representation of the body, and between the body mesh and 3D pose, we regress the mesh and 3D pose from the estimated SMPL parameters ($\widehat{\theta}, \widehat{\beta}$) and additional 3D pose from $\widehat{\mathbf{V}}_m$ with the regression matrices of the SMPL model~\cite{SMPL:2015}; let $\widehat{\mathbf{V}}_m^{\rm smpl}, \widehat{\mathbf{V}}_s^{\rm smpl}$, $\widehat{\mathbf{V}}_s^{\rm mgcn}$ denote them respectively, where {\it smpl} and {\it mgcn} indicate the terms are regressed from the prediction of SMPL and Mesh-GCN. We define a mesh set as $\widehat{\mathbf{V}}_{\rm meshes} = \{\widehat{\mathbf{V}}_m, \widehat{\mathbf{V}}_m^{\rm smpl}\}$, and a 3D pose set as $\widehat{\mathbf{V}}_{\rm poses}^{3d}=\{\widehat{\mathbf{V}}_s, \widehat{\mathbf{V}}_s^{\rm smpl}, \widehat{\mathbf{V}}_s^{\rm mgcn}\}$.

% To enable training on datasets with rich 2D poses (e.g., COCO~\cite{MSCOCO_ECCV_2014}), we have a module consisted of graph layers to predict weak perspective camera parameters from the intermediate feature of mgcn module(see ~\cite{kolotouros2019cmr} for the details) and give out 2D poses projected from the estimated 3D poses; that is $\widehat{\mathbf{V}}_{\rm poses}^{2d}=\{\widehat{\mathbf{V}}_{s2d}^{sgcn}, \widehat{\mathbf{V}}_{s2d}^{\rm smpl}, \widehat{\mathbf{V}}_{s2d}^{\rm mgcn}\}$ from the estimated 3D poses in $\widehat{\mathbf{V}}_{\rm poses}^{3d}$ respectively; similarly, {\it Skeleton-GCN} indicates being regressed from Skeleton-GCN model and {\it s2d} indicates 2D pose. 
%}
%\Note{SC: why are we doing all of these?}
 

\subsection{Loss function}
\label{subsec:loss_func}
Our loss function for training the network is
\begin{equation}
\label{loss_function}
    \mathcal{L} =  \mathcal{L}_{\rm meshes} + \mathcal{L}_{\rm poses}^{\rm 3d} + \mathcal{L}_{\rm poses}^{\rm 2d} 
    + \mathcal{L}_{\theta} + \lambda\mathcal{L}_{\beta},
\end{equation}
where $ \mathcal{L}_{\rm meshes}$, $\mathcal{L}_{\rm poses}^{\rm 3d}$, $\mathcal{L}_{\rm poses}^{\rm 2d}$ are the total losses on the estimation in $\widehat{\mathbf{V}}_{\rm meshes}$, $\widehat{\mathbf{V}}_{\rm poses}^{\rm 3d}$ and $\widehat{\mathbf{V}}_{\rm poses}^{\rm 2d}$, respectively, and $\mathcal{L}_{\theta}$ and $\mathcal{L}_{\beta}$ are the losses on $\widehat{\theta}$ and $\widehat{\beta}$. We use the $L$1 loss for $ \mathcal{L}_{\rm meshes}$ and the MSE loss for all other losses.

We observe that in the body-joint losses, $\mathcal{L}_{\rm poses}^{\rm 3d}$ and $\mathcal{L}_{\rm poses}^{\rm 2d}$, the error caused by each body joint
varies a lot. For example, the body joints on legs and arms usually have much larger error than the other parts. The intuition is that the variation for body limbs is much larger compared to torso and head.  To solve this imbalance issue, we propose a new loss function, which generalizes the focal loss~\cite{2017FocalLF} to regression tasks. Focal loss addresses class imbalance by down-weighting the loss for well-classified samples. 
We modify it based on the $L$1 loss of the target, i.e.,
$$\mathcal{L}_{fl} = -(\alpha \mathcal{L})^{\gamma} \log(1-{\rm max}(\tau, \alpha \mathcal{L})),$$
where $\mathcal{L}$ is the $L$1 loss, $\alpha$ is a factor to scale $\mathcal{L}$ to (0,1), $\tau < 1$ is a threshold that truncates $\alpha\mathcal{L}$ with a maximum value to avoid unreasonably large loss when $\alpha \mathcal{L}$ approaches 1, $(\alpha \mathcal{L})^{\gamma}$ is a factor to reduce the relative loss for well-regressed vertices with $\gamma > 0$.
%When $\mathcal{L}=0$, we have $\mathcal{L}_{fl}=0$. We update the loss of the estimated 3D pose from Mesh-GCN ($\widehat{\mathbf{V}}_s^{\rm mgcn}$) with $\mathcal{L}_{fl}$ in Eq.~\ref{loss_function}.
%We found empirically that this design achieves a desired down-weighting for training. {\HC We update the loss of the estimated 3D pose from Mesh-GCN ($\widehat{\mathbf{V}}_s^{\rm mgcn}$) with $\mathcal{L}_{fl}$ in formula ~\ref{loss_function}. We empirically set $\lambda$ \Note{do you mean $\gamma$?} as 0.1 , $\tau$ as 0.8, and the weight of this loss term as 5.0 in our experiments.}


\subsection{Scheduled sampling} Our model depends on the initial 2D joints location to extract local features for the two-layer structure. We have the ground truth 2D joints $\mathbf{V}_{s2d}$ in the training data to provide precise locations but have only estimated 2D joints $\widehat{\mathbf{V}}_{s2d}$, e.g., from HRNet, to process images in the wild. To overcome this difference between training and inference, we use scheduled sampling~\cite{bengio2015scheduled} to randomly decide whether we use $\mathbf{V}_{s2d}$ or $\widehat{\mathbf{V}}_{s2d}$ during training. For each image in the $i$-th epoch, we use the true 2D location $\mathbf{V}_{s2d}$ with probability $\epsilon_i$, or an estimate from HRNet with probability $1-\epsilon_i$. When $\epsilon_i = 1$, the model is trained solely using ground truth and when $\epsilon_i = 0$, the model is trained in the same setting as inference. We schedule the decay of $\epsilon_i$ according to an inverse sigmoid: $\epsilon_i=k/k(+{\rm exp}(i/k))$. %\Note{JVB: what do we use for k? I removed the figure, maybe we can put in suppl mat?}

%We use a schedule to decay $\epsilon_i$ as a function of $i$ itself and adopt inverse sigmoid decay here, i.e., $\epsilon_i=k/k(+{\rm exp}(i/k))$ where $k\ge1$ depends on the expected speed of decay as shown in Figure~\ref{fig:scheduled_sampling}. \Note{JVB: do we a need fig for this? I think we can omit the figure}

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.8\linewidth]{images/schedule_sampling.pdf}
%    \caption{The examples of decay schedules. %\Note{figure placeholder: we may only report experiments with sigmoid-decay and need to update this figure}
%    }
%    \label{fig:scheduled_sampling}
%\end{figure}
